Decomposition of Hypergeometric SLE and Reversibility

In this paper, we consider hypergeometric SLE process for $\kappa\in (4,8)$ and $\nu>\frac{\kappa}{2}-6$. Though the definition of hypergeometric SLE process is complicated, we show that given its hitting point on a specific boundary, its conditional law can be described by SLE$_\kappa(\underline\rho)$ process. Based on this observation, by constructing a pair of curves, we derive the reversibility of hypergeometric SLE for $\kappa\in(4,8)$ and $\nu>-2$.

==> proof.tex <==
In this section, we will prove Theorem~\ref{thm::reversibility}. We suppose $\kappa\in (2,4)$ and $\kappa'\in(4,8)$ and $\kappa'=\frac{16}{\kappa}$. Recall the coupling of $\gamma$ and $\tilde\gamma$ given in Proposition~\ref{prop::coupling}. By Theorem~\ref{thm::curve}, we have that almost surely, $\gamma$ does not hit $(y,+\infty)$. We denote by $\PP$ the corresponding probability measure and denote by $\E$ the expectation. We denote by $W$ the driving function of $\gamma$ and denote by $(g_t: t\ge 0)$ the corresponding conformal map. Recall that we define $V_t(z)$ to be the Loewner evolution for $\gamma$ in~\eqref{eqn::loewner}. Given $\gamma[0,t]$, after mapping to $\HH$ by $g_t$, we denote by $\tilde W$ the driving function of $g_t(\tilde\gamma)$ and denote by $(\tilde g_{\tilde t}: \tilde t\ge 0)$ the corresponding conformal map. We denote by $\tilde V_{\tilde t}(z)$ for the Loewner evolution for every $z\in\R$ for $g_t(\tilde\gamma)$, which is defined similarly as~\eqref{eqn::loewner}. For every $z\in (y,+\infty)$, we define $\tilde\tau(t,z)$ the hitting time of $\tilde\gamma$ at the union of $(0,x]$ and the right side of $\gamma[0,t]$ and $[z,+\infty)$. For $t\ge 0$ and $0\le \tilde t<\tilde\tau(t,z)$, we define 
\begin{align}\label{eqn::defmart}
M_{t,\tilde t}(z)=&\tilde g'_{\tilde t}(V_t(z))g'_t(z)(\tilde V_{\tilde t}(V_t(z))-\tilde V_{\tilde t}((V_t(y))^{+}))^{\frac{\kappa-4}{2}}(\tilde V_{\tilde t}(V_t(z))-\tilde W_{\tilde t})(\tilde V_{\tilde t}(V_t(z))-\tilde V_{\tilde t}((V_t(y))^{-}))^{\frac{\kappa(2+\nu)-8}{8}}\notag\\
&\times(\tilde V_{\tilde t}(V_t(z))-\tilde V_{\tilde t}(V_t(x)))^{-\frac{(2+\nu)\kappa}{8}}(\tilde V_{\tilde t}(V_t(z))-\tilde V_{\tilde t}(W_t))^{-\frac{\kappa}{4}}.
\end{align}
As in Section~\ref{sec::hyper}, by considering the absolute continuity, the Loewner flows in~\eqref{eqn::defmart} are all well-defined even after swallowing times of some marked points.
We denote by $\eta$ the $\hSLE_{\kappa'}(\nu)$ curve from $0$ to $\infty$ and denote by $\PP_{\hSLE}$ the probability measure and denote by $\E_{\hSLE}$ the correponding expectation. We define $\tau_\eps$ to be the hitting time of $\gamma$ of the $\eps$-neighbour of $[y,+\infty)$.
\begin{lemma}\label{lem::1}
If $\tilde t=0$, for $t\le \tau_\eps$, we define 
\[N_t:=\int_{y}^{+\infty}M_{t,0}(z)dz.\]
For any bounded measurable function $f$ on the curve space, we have
\[\E_{\hSLE}[f(\eta[0,\tau_\eps])]=\E\left[f(\gamma[0,\tau_\eps])\frac{N_{\tau_\eps}}{N_0}\right].\]
\end{lemma}
\begin{proof}
For $t\le \tau_\eps$, note that $\tilde W_0=V_t(y)$. Recall notations given in~\eqref{eqn::notations}. We have
\begin{align*}
M_{t,0}&=g_t'(z)(V_t(z)-V_t(y))^{\frac{6\kappa+\kappa\nu-16}{8}}(V_t(z)-V_t(x))^{-\frac{(2+\nu)\kappa}{8}}(V_t(z)-W_t)^{-\frac{\kappa}{4}}\\
&=g_t'(z)(V_t(z)-V_t(y))^{-\frac{2(\kappa'-\nu-6)}{\kappa'}}(V_t(z)-V_t(x))^{-\frac{2(2+\nu)}{\kappa'}}(V_t(z)-W_t)^{-\frac{4}{\kappa'}}
\end{align*}
By standard I\^to's formula, we know that for every $z\in [y,+\infty)$, we have $\{M_{t\wedge\tau_\eps,0}(z)\}_{t\ge 0}$ is a martingale for $\gamma$. Recall we defined $F$ in~\eqref{eqn::integral}. By direct computation, we have
\begin{align*}
N_t&=\int_{V_t(y)}^\infty (u-V_t(y))^{-\frac{2(\kappa'-\nu-6)}{\kappa'}}(u-V_t(x))^{-\frac{2(2+\nu)}{\kappa'}}(u-W_t)^{-\frac{4}{\kappa'}}du\\
&=\int_{1}^\infty u^{-\frac{\kappa'}{4}}(u-1)^{-\frac{2(\kappa'-\nu-6)}{\kappa'}}\left(u-\frac{V_t(x)-W_t}{V_t(y)-W_t}\right)^{-\frac{2(\nu+2)}{\kappa'}}du\\
&=(V_t(y)-W_t)^{\frac{4-\kappa'}{\kappa'}}F\left(\frac{V_t(x)-W_t}{V_t(y)-W_t}\right).
\end{align*}
Thus, $\{N_{t\wedge\tau_\eps}\}_{t\ge 0}$ is a martingale for $\gamma$. Thus, by Girsanov theorem, we have that weighted by $\frac{N_{\tau_\eps}}{N_0}$, the driving function of $\gamma$
satisfies the SDEs~\eqref{eqn::hyperSDE}. This completes the proof.
\end{proof}
\begin{remark}
From Theorem~\ref{thm::change}, $\{M_{t\wedge\tau_\eps,0}(z)\}_{t\ge 0}$ is the martingale to transfer the law of $\SLE_{\kappa'}(\nu+2,\kappa'-6-\nu)$ process to the law of $\SLE_{\kappa'}(\nu+2,\kappa'-6-\nu,-4)$ process with an additional marked point $z$. Thus, Lemma~\ref{lem::1} is essentially obtained from Theorem~\ref{thm::change} and Theorem~\ref{thm::decom}.
\end{remark}
\begin{lemma}\label{lem::2}
Given $\gamma[0,t]$, we denote by $\PP_{\gamma[0,t]}$ the regular conditional probability measure of $\tilde\gamma$ and denote by $\E_{\gamma[0,t]}$ the corresponding expectation. If we denote by $\tilde\tau(t)$ the hitting time of $\tilde\gamma$ at the union of $(0,x]$ and the right side of $\gamma[0,t]$and by $\tilde\tau(z)$ the hitting time of $\tilde\gamma$ at $[z,+\infty)$, 
\begin{itemize}
\item
On the event $\{\tilde\tau(t,z)=\tilde\tau(z)\}$, we define
\[M_{t,\tilde\tau(t,z)}(z):=0.\]
\item
On the event $\{\tilde\tau(t,z)=\tilde\tau(t)\}$, we define
\[M_{t,\tilde\tau(t,z)}(z):=\tilde g'_{\tilde\tau(t,z)}(V_t(z))g'_t(z)(\tilde V_{\tilde\tau(t,z)}(V_t(z))-\tilde V_{\tilde\tau(t,z)}((V_t(y))^{+}))^{\frac{\kappa-4}{2}}(\tilde V_{\tilde\tau(t,z)}(V_t(z))-\tilde V_{\tilde\tau(t,z)}(W_t))^{-\frac{\kappa}{4}}.\]
\end{itemize}
Then, we have that $\{M_{t,\tilde t\wedge\tilde\tau(t,z)}\}_{\tilde t \ge 0}$ is a martingale for $\tilde\gamma$ under $\PP_{\gamma[0,t]}$.
\end{lemma}
\begin{proof}
%Recall that we denote by $\LC$ the unbounded connected component  as in Proposition~\ref{prop::coupling}. 
By Proposition~\ref{prop::coupling}, $g_t(\tilde\gamma)$ has the same law as the $\SLE_\kappa\left(\frac{\kappa}{4}(2+\nu)-2,-\frac{\kappa}{4}(2+\nu),-\frac{\kappa}{2};\kappa-4\right)$ from $V_t(y)$ with marked points $x_3^L=W_t$, $x_2^L=V_t(x)$, $x_1^L=(V_t(y))^-$ and $x_1^R=(V_t(y))^+$. For every $\eps>0$, we define $\tilde\tau(t,z,\eps)$ to be the hitting time of $\tilde\gamma$ at the union of $(0,x]$ and the right side of $\gamma[0,t]$ and the $\eps$-neighbour of $[z,+\infty)$. By standard I\^to's formula, we know that for every $z\in [y,+\infty)$, we have that $\{M_{t,\tilde t\wedge\tilde\tau(t,z,\eps)}\}_{\tilde t \ge 0}$ is a martingale for $\tilde\gamma$ under $\PP_{\gamma[0,t]}$. Thus, $\{M_{t,\tilde t}:\tilde t<\tilde\tau(t,z)\}$ is a local martingale. Next, we prove that $\{M_{t,\tilde t\wedge\tilde\tau(t,z)}\}_{\tilde t \ge 0}$ is a martingale.

%On the event $\{\tilde\tau(t,z)=\tilde\tau(z)\}$,  by Proposition~\ref{prop::property}, we may assume that $\tilde\gamma$ hits $[z,+\infty)$ at $w\in(z,+\infty)$. Since $\kappa\in (2,4)$, we have 
%\begin{equation}\label{eqn::1}
%(\tilde V_{\tilde t}(V_t(z))-\tilde V_{\tilde t}((V_t(y))^{+}))^{\frac{\kappa-2}{2}}\to 0,\quad\text{as }t\to \tilde\tau(z)
%\end{equation}
%Note that for $r\in (y,+\infty)$, we have $\tilde g''_t(V_t(r))\le 0$ before the hitting time of $\tilde\gamma$ at $(y,+\infty)$. This implies that for $r\in (z,w)$, we have $\tilde g_t'(V_t(z))\le \tilde g_t'(V_t(r))$ before $\tilde\tau(z)$. Thus, we have
%\[\tilde g_t'(V_t(z))\le 2\frac{\tilde V_{\tilde t}(V_t\left(\frac{w+z}{2}\right))-\tilde V_{\tilde t}(V_t(z))}{w-z}.\]
%By standard argument (for instance, see~\cite{}), there exists $C>0$ such that
%\begin{equation}\label{eqn::2}
%\frac{\tilde g_t'(V_t(z))}{\tilde V_{\tilde t}(V_t(z))-\tilde V_{\tilde t}((V_t(y))^{+})}\le \frac{2}{w-z}\times\frac{\tilde V_{\tilde t}(V_t\left(\frac{w+z}{2}\right))-\tilde V_{\tilde t}(V_t(z))}{\tilde V_{\tilde t}(V_t(z))-\tilde V_{\tilde t}((V_t(y))^{+})}\le C\times \frac{2}{w-z}.
%\end{equation}
%Plugging~\eqref{eqn::1} and~\eqref{eqn::2} into~\eqref{eqn::defmart}, we derive the first item. 
On the event $\{\tilde\tau(t,z)=\tilde\tau(t)\}$, note that
\[\tilde V_{\tilde t}((V_t(y))^{-})\to \tilde W_{\tilde\tau(t)},\quad \tilde V_{\tilde t}(V_t(x))\to \tilde W_{\tilde\tau(t)},\quad \tilde W_{\tilde t}\to \tilde W_{\tilde\tau(t)},\quad\text{as }\tilde t\to \tilde\tau(t).\]
Thus, we have $M_{t,\tilde t\wedge\tilde\tau(t,z)}\to M_{t,\tilde\tau(t,z)}$ as $\tilde t\to\infty$ on the event $\{\tilde\tau(t,z)=\tilde\tau(t)\}$.

In the remaining proof, we will use the same strategy as in~\cite[Proposition 3.6]{WuHyperSLE}. Note that by Girsanov theorem, weighted by $\left\{\frac{M_{t,\tilde t\wedge\tilde\tau(t,z,\eps)}}{M_{t,0}}\right\}_{\tilde t \ge 0}$, the law of $g_t(\tilde\gamma[0,\tilde\tau(t,z,\eps)])$ is the same as the law of 
\\$\SLE_\kappa\left(\frac{\kappa}{4}(2+\nu)-2,-\frac{\kappa}{4}(2+\nu),-\frac{\kappa}{2};\kappa-4,\kappa\right)$ curve with  marked points $x_1^L=(V_t(y))^-$, $x_2^L=V_t(x)$, $x_3^L=W_t$  and $x_1^R=(V_t(y))^+$, $x_2^R=V_t(z)$, which stops at the corresponding stopping time. We denote the $\SLE_\kappa\left(\frac{\kappa}{4}(2+\nu)-2,-\frac{\kappa}{4}(2+\nu),-\frac{\kappa}{2};\kappa-4,\kappa\right)$ curve by $\hat{\gamma}_z$ and denote by the probability measure of $\hat{\gamma}_z$ by $Q^z_{\gamma[0,t]}$. Note that by Theorem~\ref{thm::curve}, almost surely, $\hat{\gamma}_z$ does not hit $(V_t(z),+\infty)$. By Lemma~\ref{lem::aux}, $\hat{\gamma}_z$ does not hit $V_t(z)$ as well. 
%Note that
%\[d(\tilde V_{\tilde t}(V_t(z))-\tilde V_{\tilde t}(W_t))=\frac{2d\tilde t}{\tilde V_{\tilde t}(V_t(z))-\tilde W_{\tilde t}}-\frac{2d\tilde t}{\tilde V_{\tilde t}(W_t)-\tilde W_{\tilde t}}\ge 0.\]
%Thus, we have
%\begin{equation}\label{eqn::aux11}
%\tilde V_{\tilde t}(V_t(z))-\tilde V_{\tilde t}(W_t)\ge V_t(z)-W_t.
%\end{equation}
For every $\eps>0$,  we define $\tilde\tau_\eps$ to be the hitting time of $\tilde\gamma$ at the $\eps$-neighbour of $[V_t(z),+\infty)$ and define the event $\tilde A_\eps:=\{\tilde\tau_\eps\ge \tilde\tau(t)\}$. Define the event $\hat A_\eps$ similarly for $\hat{\gamma}_z$. Then, note that on event $\tilde A_\eps:=\{\tilde\tau_\eps\ge \tilde\tau(t)\}$, we have $\{\tilde\tau(t,z)=\tilde\tau(t)\}$ and there exists a constant $C=C(\eps)$ such that 
\[M_{t,\tilde t\wedge \tilde\tau(t,z)}\le C,\quad\text{for every }\tilde t>0.\] 
Thus, by dominated convergence theorem, if we fix $\tilde t_0>0$ and for every bounded measurable function $f$ on the curve space, we have
\begin{align*}
Q^z_{\gamma[0,t]}[f(\hat{\gamma}_z[0,\tilde t_0\wedge\tilde\tau(t,z)])\one_{\hat A_\eps}]&=\E_{\gamma[0,t]}\left[f(\tilde\gamma[0,\tilde t_0\wedge\tilde\tau(t,z)])\one_{\tilde A_\eps}\frac{M_{t,\tilde t_0\wedge\tilde\tau(t,z)}}{M_{t,0}}\right]\\
&=\lim_{\tilde t\to\infty}\E_{\gamma[0,t]}\left[f(\tilde\gamma[0,\tilde t_0\wedge\tilde\tau(t,z)])\one_{\tilde A_\eps}\frac{M_{t,\tilde t\wedge\tilde\tau(t,z)}}{M_{t,0}}\right]\\
&=\E_{\gamma[0,t]}\left[f(\tilde\gamma[0,\tilde t_0\wedge\tilde\tau(t,z)])\one_{\tilde A_\eps}\frac{M_{t,\tilde\tau(t,z)}}{M_{t,0}}\right].
\end{align*}
Recall that we defined $M_{t,\tilde\tau(t,z)}=0$ on the event $\{\tilde\tau(t,z)=\tilde\tau(z)\}$. By letting $\eps\to 0$, combining the fact that $\hat{\gamma}_z$ does not hit $[V_t(z),\infty)$, if we define $\hat\tau(t)$ to be the hitting time of $\hat\gamma_z$ at the union of $(0,x]$ and the right side of $\gamma[0,t]$, we have
\begin{align*}
&\E_{\gamma[0,t]}\left[f(\tilde\gamma[0,\tilde t_0\wedge\tilde\tau(t,z)])\frac{M_{t,\tilde\tau(t,z)}}{M_{t,0}}\right]\\
=&Q^z_{\gamma[0,t]}[f(\hat{\gamma}_z[0,\tilde t_0\wedge\hat\tau(t)])]\\
=&\E_{\gamma[0,t]}\left[f(\tilde\gamma[0,\tilde t_0\wedge\tilde\tau(t,z)])\frac{M_{t,\tilde t_0\wedge\tilde\tau(t,z)}}{M_{t,0}}\right]-\lim_{\eps\to 0} \E_{\gamma[0,t]}\left[f(\tilde\gamma[0,\tilde t_0\wedge\tilde\tau(t,z)])\one_{{\tilde A_\eps}^c}\frac{M_{t,\tilde t_0\wedge\tilde\tau(t,z)}}{M_{t,0}}\right].
\end{align*}
By taking $f=1$, we have that
\[\lim_{\eps\to 0} \E_{\gamma[0,t]}\left[\one_{{\tilde A_\eps}^c}\frac{M_{t,\tilde t_0\wedge\tilde\tau(t,z)}}{M_{t,0}}\right]=0.\]
This implies that
\begin{equation}\label{eqn::RNderi}
Q^z_{\gamma[0,t]}[f(\hat{\gamma}_z[0,\tilde t_0\wedge\hat\tau(t)])]=\E_{\gamma[0,t]}\left[f(\tilde\gamma[0,\tilde t_0\wedge\tilde\tau(t,z)])\frac{M_{t,\tilde\tau(t,z)}}{M_{t,0}}\right]
=\E_{\gamma[0,t]}\left[f(\tilde\gamma[0,\tilde t_0\wedge\hat\tau(t)])\frac{M_{t,\tilde t_0\wedge\tilde\tau(t,z)}}{M_{t,0}}\right].
\end{equation}
Thus, we have that $\{M_{t,\tilde t\wedge\tilde\tau(t,z)}\}_{\tilde t \ge 0}$ is a martingale and $\hat{\gamma}_z$ is absolutely conintinuous with respect to $\tilde\gamma$. This completes the proof.
\end{proof} 
%\begin{remark}
%From Theorem~\ref{thm::change}, $\{M_{t,\tilde t\wedge\tilde\tau(t,z)}\}_{\tilde t \ge 0}$ is the martingale to transfer the law of 
%\\
%$\SLE_\kappa\left(\frac{\kappa}{4}(2+\nu)-2,-\frac{\kappa}{4}(2+\nu),-\frac{\kappa}{2};\kappa-4\right)$ process to the law of $\SLE_\kappa\left(\frac{\kappa}{4}(2+\nu)-2,-\frac{\kappa}{4}(2+\nu),-\frac{\kappa}{2};\kappa-4,\kappa\right)$ with additional marked point $z$. Thus, Lemma~\ref{lem::2} is essentially obtained from Theorem~\ref{thm::change}.
%\end{remark}
Recall that we denote by $\tau_\eps$  the hitting time of $\gamma$ of the $\eps$-neighbour of $[y,+\infty)$ and denote by $\tilde\tau(t,z)$ the hitting time of $\tilde\gamma$ at the union of $(0,x]$ and the right side of $\gamma[0,t]$ and $[z,+\infty)$ for $z\in (y,+\infty)$. Now, we define the probability measure $\LQ_\eps$ to be the probablity measure of $\PP$ weighted by $\frac{\int_{y}^{\infty}M_{\tau_\eps,\tilde\tau(\tau_\eps,z)}dz}{N_0}$.
\begin{lemma}\label{lem::3}
Under the probability measure $\LQ_\eps$, the marginal law of $\gamma[0,\tau_\eps]$ is the same as the law of $\hSLE_{\kappa'}(\nu)$ with force points $x$, $y$ stopped at the hitting time at the $\eps$-neighbour of $[y,\infty)$. The law of $\gamma[0,\tau_\eps]$ given $\tilde\gamma$ can be described by the following way: We first generate $\tilde\gamma$ under the probability measure $\LQ_\eps$. Denote by $\LD$ the unbounded connected component of $\HH\setminus\tilde\gamma$. Then, $\gamma$ has the same law as the $\SLE_{\kappa'}$ curve stopped at the hitting time at the $\eps$-neighbour of $[y,\infty)$.%Suppose $f$ and $g$ are two bounded measurable functions on curve space. Then, we have
%\[\LQ_\eps[f(\gamma[0,\tau_\eps])g(\tilde\gamma)]=.\]
\end{lemma}
\begin{proof}
The first statement is obtained from Lemma~\ref{lem::1} and Lemma~\ref{lem::2} directly. It suffices to prove the second statement. We denote by $\tilde\tau$ the hitting time of $\tilde\gamma$ at $(0,x]$. 
Suppose $f$ and $g$ are positive measuable functions on the curve space. We denote by $\psi_{t,\tilde t}$ the conformal map from the unbounded component of $\HH\setminus (\gamma[0,t]\cup\tilde\gamma[0,\tilde t])$ onto $\HH$ such that 
\[\psi_{t,\tilde t}(z)=z+o(1),\quad\text{as }z\to\infty.\]
We denote by $\tilde\tau(\tau_\eps)$ the hitting time of $\tilde\gamma$ at $(0,x]$ and the right side of $\gamma[0,\tau_\eps]$. 
Recall that we denote by $(\tilde g_{\tilde t}: \tilde t\ge 0)$ the conformal map associated with $\tilde\gamma$. We denote by $W_{\tilde\gamma,\cdot}$ the driving function of $\tilde g_{\tilde\tau}(\gamma)$ and denote by $(g_{\tilde\gamma,t}:t\ge 0)$ the corresponding conformal map. Note that 
\[\psi_{\tau_\eps,\tilde\tau(\tau_\eps)}=\psi_{\tau_\eps,\tilde\tau}.\] Thus, we have
\begin{equation}\label{eqn::compconformal}
\psi_{\tau_\eps,\tilde\tau(\tau_\eps)}=g_{\tilde\gamma,\tau_\eps}\circ\tilde g_{\tilde\tau}.
\end{equation}
We define  $w_{\tilde\gamma}:=\max\{r:r\in\tilde\gamma\cap[y,+\infty)\}$. Recall the definition of $M_{\tau_\eps,\tilde\tau(\tau_\eps,z)}$ given in Lemma~\ref{lem::2}, we have
\begin{align}\label{eqn::finallyform}
&M_{\tau_\eps,\tilde\tau(\tau_\eps,z)}\notag\\
=&\one_{\{\tilde\tau(\tau_\eps,z)=\tilde\tau(\tau_\eps)\}}\tilde g'_{\tilde\tau(\tau_\eps,z)}(V_{\tau_\eps}(z))g'_{\tau_\eps}(z)(\tilde V_{\tilde\tau({\tau_\eps},z)}(V_{\tau_\eps}(z))-\tilde V_{\tilde\tau({\tau_\eps},z)}((V_{\tau_\eps}(y))^{+}))^{\frac{\kappa-4}{2}}(\tilde V_{\tilde\tau({\tau_\eps},z)}(V_{\tau_\eps}(z))-\tilde V_{\tilde\tau({\tau_\eps},z)}(W_{\tau_\eps}))^{-\frac{\kappa}{4}}\notag\\
=&\one_{\{\tilde\tau(\tau_\eps,z)=\tilde\tau(\tau_\eps)\}}\psi'_{\tau_\eps,\tilde\tau(\tau_\eps)}(z)(\psi_{\tau_\eps,\tilde\tau(\tau_\eps)}(z)-\psi_{\tau_\eps,\tilde\tau(\tau_\eps)}(w_{\tilde\gamma}))^{\frac{\kappa-4}{2}}(\psi_{\tau_\eps,\tilde\tau(\tau_\eps)}(z)-\psi_{\tau_\eps,\tilde\tau(\tau_\eps)}(\gamma(\tau_\eps)))^{-\frac{\kappa}{4}}
\end{align}
Combining with~\eqref{eqn::compconformal} and~\eqref{eqn::finallyform}, we have
\begin{align}\label{eqn::jointlaw}
&\LQ_\eps[f(\gamma[0,\tau_\eps])g(\tilde\gamma)]\notag\\
=&\frac{1}{N_0}\int_{y}^\infty \E[f(\gamma[0,\tau_\eps])g(\tilde\gamma)M_{\tau_{\eps},\tilde\tau(\tau_\eps,z)}(z)]dz\notag\\
=&\frac{1}{N_0}\E\left[f(\gamma[0,\tau_\eps])g(\tilde\gamma)\int_{w_{\tilde\gamma}}^{\infty}\psi'_{\tau_\eps,\tilde\tau(\tau_\eps)}(z)(\psi_{\tau_\eps,\tilde\tau(\tau_\eps)}(z)-\psi_{\tau_\eps,\tilde\tau(\tau_\eps)}(w_{\tilde\gamma}))^{\frac{\kappa-4}{2}}(\psi_{\tau_\eps,\tilde\tau(\tau_\eps)}(z)-\psi_{\tau_\eps,\tilde\tau(\tau_\eps)}(\gamma(\tau_\eps)))^{-\frac{\kappa}{4}}dz\right]\notag\\
=&\frac{B\left(1-\frac{\kappa}{4},\frac{\kappa-2}{2}\right)}{N_0}\E\left[f(\gamma[0,\tau_\eps])g(\tilde\gamma)(g_{\tilde\gamma,\tau_\eps}(\tilde g_{\tilde\tau}(w_{\tilde\gamma}))-W_{\tilde\gamma,\tau_\eps})^{\frac{\kappa-4}{4}}\right]\notag\\
=&\frac{B\left(1-\frac{\kappa}{4},\frac{\kappa-2}{2}\right)}{N_0}\E\left[g(\tilde\gamma)N_{\tilde\gamma, 0}\E_{\tilde\gamma}\left[f(\gamma[0,\tau_\eps])\frac{N_{\tilde\gamma,\tau_\eps}}{N_{\tilde\gamma,0}}\right]\right],
\end{align}
where $B\left(\cdot,\cdot\right)$ is the Beta function and we denote $\E_{\tilde\gamma}$ by the conditional expectation of $\gamma$ given $\tilde\gamma$ and we define
\[N_{\tilde\gamma,t}:=(g_{\tilde\gamma,t}(\tilde g_{\tilde\tau}(w_{\tilde\gamma}))-W_{\tilde\gamma,t})^{\frac{\kappa-4}{4}}=(g_{\tilde\gamma,t}(\tilde g_{\tilde\tau}(w_{\tilde\gamma}))-W_{\tilde\gamma,t})^{\frac{4-\kappa'}{\kappa'}}.\]
Recall that by Proposition~\ref{prop::coupling}, we have the conditional law of $\gamma$ given $\tilde\gamma$ is the same as the law of $\SLE_{\kappa'}(\kappa'-4)$ curve in the unbounded connected component of $\HH\setminus\tilde\gamma$ from $0$ to $\infty$. More precisely, we have
\[dW_{\tilde\gamma,t}=\sqrt{\kappa'}B_t+\frac{\kappa'-4}{W_{\tilde\gamma,t}-g_{\tilde\gamma,t}(\tilde g_{\tilde\tau}(w_{\tilde\gamma}))}dt,\]
where $B_t$ is a one-dimensional Brownian motion. By I\^to's formula, we have that $\{N_{\tilde\gamma,t}\}_{t\ge 0}$ is a martingale for $\gamma$ under $\E_{\tilde\gamma}$. By Girsanov's theorem, under $\E_{\tilde\gamma}$, weightded by $\left\{\frac{N_{\tilde\gamma,t}}{N_{\tilde\gamma,0}}\right\}_{t\ge 0}$, the law of $\gamma[0,\tau_\eps]$ is the same as the law of $\SLE_{\kappa'}$ stopped at the corresponding stopping time. This completes the proof.
\end{proof}
In the next Lemma, we will give an expression of the marginal law of $\tilde\gamma$ under $\LQ_\eps$. Suppose $l$ has the law of $\SLE_\kappa\left(\frac{\kappa}{4}(2+\nu)-2,\frac{\kappa}{4}(2+\nu);\kappa-4\right)$  with marked points $x_1^L=y-$, $x_2^L=x$ and $x_1^R=y^+$. We denote by $\PP_l$ the law of $l$ and by $\E_l$ the corresponding expectation. Denote by $\tau_l$ the hitting time of $l$ at $(-\infty,x]$. Denote by $W_{l,\cdot}$ the driving function of $l$ and by $\{g_{l,t}: 0\le t\le \tau_l\}$ the corresponding conformal map. Denote by $V_{l,\cdot}$ the corresponding Loewner evolution.
\begin{lemma}\label{lem::4}
Recall that we denote by $\tilde\tau$ the hitting time of $\tilde\gamma$ at $(0,x]$. Then, suppose that $g$ is a bounded and measurable function on the curve space $\LC$, we have
\[\LQ_\eps[g(\tilde\gamma[0,\tilde\tau])]=\frac{1}{\mathcal{Z}}\E_l[g(l[0,\tau_l])(g'_{l,\tau_l}(0))^{\frac{3\kappa-8}{16}}\one_{\{l\cap(-\infty,0]=\emptyset\}}],\]
where $\mathcal{Z}$ is a constant. 
\end{lemma}
\begin{proof}
First of all, by~\cite[Theorem 3]{SchrammWilsonSLECoordinatechanges}, $l$ has the same law as $\SLE_\kappa\left(\frac{\kappa}{4}(2+\nu)-2;\kappa-4\right)$ curve form $y$ to $x$ stopped at its hitting time at $(-\infty,x)$. Thus, we have almost surely, $l$ ends at $(-\infty,x)$ and $l$ does not hit $0$ and $z$ for every fixed $z\in (y,+\infty)$.

For $z\in (y,+\infty)$, we define $\tau_l(z,0)$ to be the hitting time of $(-\infty,0]\cup [z,+\infty)$. For $t<\tau_l(z,0)\wedge \tau_l$, we define
\begin{align*}
R_t(z):=&g'_{l,t}(z)g'_{l,t}(0)^{\frac{3\kappa-8}{16}}(V_{l,t}(z)-W_{l,t})(V_{l,t}(z)-V_{l,t}(y^-))^{\frac{\kappa(2+\nu)-8}{8}}(V_{l,t}(z)-V_{l,t}(y^+))^{\frac{\kappa-4}{2}}(V_{l,t}(z)-V_{l,t}(x))^{-\frac{(2+\nu)\kappa}{8}}\\
&\times (V_{l,t}(z)-V_{l,t}(0))^{-\frac{\kappa}{4}}(V_{l,t}(0)-W_{l,t})^{-\frac{1}{2}}(V_{l,t}(0)-V_{l,t}(y^-))^{\frac{8-\kappa(2+\nu)}{16}}(V_{l,t}(0)-V_{l,t}(y^+))^{\frac{4-\kappa}{4}}\\
&\times(V_{l,t}(0)-V_{l,t}(x))^{\frac{(2+\nu)\kappa}{16}}.
\end{align*}
We define $\tau_{l,\eps}(z,0)$ to be the first time that $l$ hits the $\eps$-neighbour of $(-\infty,0]\cup [z,+\infty)$ and define $\tau_{l,\eps}$ the first time that $l$ hits the $\eps$-neighbour of $(-\infty,x]$. By I\^to's formula, we have $\{R_{t\wedge\tau_{l,\eps}(z,0)\wedge\tau_{l,\eps}}\}_{t\ge 0}$ is a martingale for $l$. 
By Girsanov's theorem, weighted by $\left\{\frac{R_{t\wedge\tau_{l,\eps}(z,0)\wedge\tau_{l,\eps}}(z)}{R_0(z)}\right\}_{t\ge 0}$, the law of $l[0,\tau_{l,\eps}(z,x)\wedge\tau_{l,\eps}]$ is same as the law of  $\SLE_\kappa\left(\frac{\kappa}{4}(2+\nu)-2,-\frac{\kappa}{4}(2+\nu),-\frac{\kappa}{2};\kappa-4,\kappa\right)$ curve with  marked points $x_1^L=y^-$, $x_2^L=x$, $x_3^L=0$  and $x_1^R=y^+$, $x_2^R=z$, which stopped at the corresponding stopping time. As in the proof of Lemma~\ref{lem::2}, we denote the $\SLE_\kappa\left(\frac{\kappa}{4}(2+\nu)-2,-\frac{\kappa}{4}(2+\nu),-\frac{\kappa}{2};\kappa-4,\kappa\right)$ curve by $\hat{\gamma}_z$. By Lemma~\ref{lem::aux}, we know that almost surely, $\hat{\gamma}_z$ does not hit $z$ and $0$. By the same argument as in Lemma~\ref{lem::2}, 
\begin{itemize}
\item
On the event $\{\tau_{l}(z,0)\le\tau_l\}$, we define $R_{\tau_{l}(z,0)\wedge\tau_l}(z):=0$.
\item
On the event $\{\tau_{l}(z,0)>\tau_l\}$, we define
\begin{align}\label{eqn::auxmart}
R_{\tau_{l}(z,0)\wedge\tau_l}(z):=&g_{l,\tau_l}'(z)g_{l,\tau_l}'(0)^{\frac{3\kappa-8}{16}}(V_{l,\tau_l}(z)-V_{l,\tau_l}(y^+))^{\frac{\kappa-4}{2}}(V_{l,\tau_l}(z)-V_{l,\tau_l}(0))^{-\frac{\kappa}{4}}(V_{l,\tau_l}(0)-V_{l,\tau_l}(y^+))^{\frac{4-\kappa}{4}}.
\end{align}
\end{itemize}
then we have that $\left\{R_{t\wedge\tau_{l}\wedge \tau_{l}(z,0)}(z)\right\}_{t\ge 0}$ is a martingale. Recall that in the proof of Lemma~\ref{lem::2}, we denote by $Q^z$ the law of $\hat{\gamma}_z$. (We omit the subscript $\gamma[0,t]$ since here we assume $t=0$.) We denote by $\hat\tau$ the hitting time of $\hat\gamma$ at $(0,x]$. Then, by~\eqref{eqn::RNderi} and letting $\tilde t_0\to\infty$, we have
\[\E_l\left[g(l)\frac{R_{\tau_{l}(z,0)\wedge\tau_l}(z)}{R_0(z)}\right]=Q^z[g(\hat\gamma_z[0,\hat\tau])]=\E\left[g(\tilde\gamma[0,\tilde\tau(0,z)])\frac{M_{0,\tilde\tau(0,z)}(z)}{M_{0,0}(z)}\right].\]
%We define
%\[\tilde N_{t}:=\int_{y}^{\infty}R_{t\wedge\tau_{l}\wedge \tau_{l}(z,0)}(z)dz\]
%Then, $\{\tilde N_t\}_{t\ge 0}$ is a martingale.
%Note that by definition
%\[N_{\tau_l}=g_t'(0)^{\frac{3\kappa-8}{16}}B\left(1-\frac{\kappa}{4},\frac{\kappa-2}{2}\right),\]
%where $B(\cdot,\cdot)$ is the Beta function as before.
Note that by definition, we have that $\frac{R_0(z)}{M_{0,0}(z)}$ is independent of $z$. Recall that we denote by $B(\cdot,\cdot)$ the Beta function. Then, we have
\begin{align*}
&\E_l[g(l[0,\tau_l])(g'_{l,\tau_l}(0))^{\frac{3\kappa-8}{16}}\one_{\{l\cap(-\infty,0]=\emptyset\}}]\\
=&\frac{1}{B\left(1-\frac{\kappa}{4},\frac{\kappa-2}{2}\right)}\int_{y}^{\infty}\E_l\left[g(l)R_{\tau_{l}(z,0)\wedge\tau_l}(z)\right]dz\\
=&\frac{1}{B\left(1-\frac{\kappa}{4},\frac{\kappa-2}{2}\right)}\int_{y}^{\infty}\E\left[g(\tilde\gamma[0,\tilde\tau(0,z)])\frac{M_{0,\tilde\tau(0,z)}(z)R_0(z)}{M_{0,0}(z)}\right]dz\\
=&\frac{R_0(z)}{M_{0,0}(z)B\left(1-\frac{\kappa}{4},\frac{\kappa-2}{2}\right)}\int_{y}^{\infty}\E\left[g(\tilde\gamma[0,\tilde\tau(0,z)])M_{0,\tilde\tau(0,z)}(z)\right]dz\\
=&{\mathcal{Z}}\LQ_\eps[g(\tilde\gamma[0,\tilde\tau])],
\end{align*}
where the last equation is obtained by taking $f=1$ in~\eqref{eqn::jointlaw}.
This completes the proof.
\end{proof}
Now, we come to the proof of Theorem~\ref{thm::reversibility}.
\begin{proof}[Proof of Theorem~\ref{thm::reversibility}]
In this proof, we will use the same notations as in Lemma~\ref{lem::1}, Lemma~\ref{lem::2}, Lemma~\ref{lem::3}  and Lemma~\ref{lem::4}. We define $\tau$ to be the hitting time of $\gamma$ at $(y,+\infty)$. Note that by Lemma~\ref{lem::3} and Lemma~\ref{lem::4}, the joint law of $(\gamma[0,\tau],\tilde\gamma[0,\tilde\tau])$ under $\{\LQ_\eps\}_{\eps>0}$ is consistent. Thus, we can define the a probability measure $\LQ$ such that the law of $(\gamma[0,\tau_\eps],\tilde\gamma[0,\tilde\tau])$ are the same under $\LQ_\eps$ and $\LQ$. Then, since $\hSLE_{\kappa'}(\nu)$ is a continuous curve, by Lemma~\ref{lem::3}, we have that the marginal law of $\gamma[0,\tau]$ is same as the law of $\hSLE_{\kappa'}(\nu)$ stopped at the hitting time at $(y,+\infty)$. Define $w:=\min\{r:r\in [x,y]\cap\tilde\gamma[0,\tilde\tau]\}$. Now, we define the coupling of $(\gamma,\tilde\gamma)$ such that the joint law of $(\gamma[0,\tau],\tilde\gamma[0,\tilde\tau])$ is same as $\LQ$, after sampling $(\gamma[0,\tau],\tilde\gamma[0,\tilde\tau])$, the remaining curve $\gamma[\tau,+\infty)$ evolves as an independent $\SLE_{\kappa'}$ from $\gamma(\tau)$ to $\infty$, in the unbounded connected componnent of $\HH\setminus((\gamma[0,\tau]\cup\tilde\gamma[0,\tilde\tau]))$; and $\tilde\gamma[\tilde\tau,\infty)$ evolves as an independent $\SLE_{\kappa}(\frac{\kappa}{4}(2+\nu)-2;\kappa-4)$ from $\tilde\gamma(\tilde\tau)$ to $x$ with marked points $x_1^L=w$ and $x_1^R=(\tilde\gamma(\tilde\tau))^+$, in the connected componnent of $\HH\setminus((\gamma[0,\tau]\cup\tilde\gamma[0,\tilde\tau]))$ which contains $x$ on its boundary. We still denote this coupling by $\LQ$. 

Suppose $\psi:\HH\to\HH$ is an anti-conformal map from $\HH$ onto $\HH$ and $\psi(0)=\infty$ and $\psi(\infty)=0$. Note that there exists a constant $\lambda>0$ such that $\psi(z)=\frac{\lambda}{\overline z}$. We can define $\overline\LQ$ similarly as $\LQ$ by replacing $x$ by $\psi(y)$ and replacing $y$ by $\psi(x)$. We denote by the corresponding to curves by $\overline\gamma$ and $\overline{\tilde\gamma}$. It suffices to show that $\psi(\gamma)$ has the same law as $\overline\gamma$. 

We first show that $\psi(\tilde\gamma)$ has the same law as $\overline{\tilde\gamma}$. We denote by $\tilde l$ the $\SLE_\kappa\left(\frac{\kappa}{4}(2+\nu)-2,\kappa-4\right)$ curve form $y$ to $x$ with marked points $x_1^L=y^-$ and $x_1^R=y^+$. By~\cite[Theorem 3]{SchrammWilsonSLECoordinatechanges}, $l$ has the same law as $\tilde l$ stopped at its hitting time at $(-\infty,x)$. By Theorem~\ref{thm::slerever} ($\rho_1^L=\frac{\kappa}{4}(2+\nu)-2$, $\rho_1^R=\kappa-4$), we know that $\psi(\tilde l)$ has the same law as
the $\SLE_\kappa\left(\frac{\kappa}{4}(2+\nu)-2,\kappa-4\right)$ curve form $\psi(x)$ to $\psi(y)$ with marked points $x_1^L=(\psi(x))^-$ and $x_1^R=(\psi(x))^+$. Recall that in Lemma~\ref{lem::3}, $g_{l,\tau_l}$ equals to the conformal map $\phi_{\tilde l}$ from the unbounded connected component of $\HH\setminus\tilde l$ onto $\HH$, with the normalization
\[\phi_{\tilde l}(z)=z+o(1),\quad\text{as }z\to\infty.\]
For the curve $\psi(\tilde l)$, the corresponding conformal map $\phi_{\psi(\tilde l)}$ can be constructed from $\phi_{\tilde l}$ as
\[\phi_{\psi(\tilde l)}:=\frac{\lambda \overline{\phi'_{\tilde l}(0)}}{(\overline{\phi_{\tilde l}-\phi_{\tilde l}(0))}\circ\psi^{-1}}=\frac{\lambda{\phi'_{\tilde l}(0)}}{(\overline{\phi_{\tilde l}-\phi_{\tilde l}(0))}\circ\psi^{-1}},\]
where the second equality is obtained from the fact that $\phi'_{\tilde l}(0)>0$.
In particular, we have
\[\phi'_{\psi(\tilde l)}(0)=\phi'_{\tilde l}(0).\]
By Lemma~\ref{lem::4}, we show that $\psi(\tilde\gamma)$ has the same law as $\overline{\tilde\gamma}$.

We denote by $\LD$ the unbounded connected component of $\HH\setminus\tilde\gamma$ and denote by $\overline\LD$ the unbounded connected component of $\HH\setminus\overline{\tilde\gamma}$. Then we have $\psi(\tilde\gamma\cap\partial\LD)$ has the same law as $\overline{\tilde\gamma}\cap\partial\overline\LD$. By Lemma~\ref{lem::3},
given $\tilde\gamma$, the curve $\gamma$ has the same law as $\SLE_{\kappa'}$ from $0$ to $\infty$ in $\LD$. By Theorem~\ref{thm::slerever} ($\rho_1^L=\rho_1^R=0$), we have that $\psi(\gamma)$ has the same law as $\SLE_{\kappa'}$ from $0$ to $\infty$ in $\psi(\LD)$. This implies that $\psi(\gamma)$ has the same law as $\overline\gamma$.
This completes the proof.
\end{proof}  


==> proof1.tex <==
In this section, we consider the case $\frac{\kappa'}{2}-6<\nu<-2$. The proof is similar (and easier) to the proof of the case $\nu>-2$. The main difference in this case is that we need to use the coupling of flow line and counterflow line in the second item in Proposition~\ref{prop::coupling}. 
We denote by $\PP$ the corresponding probability measure and denote by $\E$ the expectation. We denote by $W$ the driving function of $\gamma$ and denote by $(g_t: t\ge 0)$ the corresponding conformal map. Recall that we define $V_t(z)$ to be the Loewner evolution for $\gamma$ in~\eqref{eqn::loewner}. For every $t>0$, we denote by $\tilde\tau_{\gamma[0,t]}$ the first time that $\tilde\gamma$ enters the unbounded connected component of $\HH\setminus\gamma[0,t]$. Recall that by Proposition~\ref{prop::property}, $\tilde\gamma$ ends at $y$. We denote by $\tilde\tau$ the hitting time of $\tilde\gamma$ at $y$. In Proposition~\ref{prop::coupling}, we derive the conditional law of $\tilde\gamma$ given $\gamma[0,t]$. By Theorem~\ref{thm::curve}, we have that $\tilde\gamma$ does not hit the left side of $\gamma$. Given $\gamma[0,t]$, after mapping to $\HH$ by $g_t$, we denote by $\tilde W_{\gamma[0,t],\cdot}$ the driving function of $g_t(\tilde\gamma[\tilde\tau_{\gamma[0,t]},\tilde\tau])$ and denote by $(\tilde g_{\gamma[0,t],\tilde t}: 0\le \tilde t\le\tilde\tau)$ the corresponding conformal map. We denote by $\tilde V_{\gamma[0,t],\tilde t}(z)$ for the Loewner evolution for every $z\in\R$ for $g_t(\tilde\gamma[\tilde\tau_{\gamma[0,t]},\tilde\tau])$, which is defined similarly as~\eqref{eqn::loewner}. For $t\ge 0$ and $0\le \tilde t\le \tilde\tau$, we define 
\begin{align}\label{eqn::defmart}
M_{t,\tilde t}(z)=&\tilde g'_{\gamma[0,t],\tilde t}(V_t(z))g'_t(z)(\tilde V_{\tilde t}(V_t(z))-\tilde V_{\tilde t}((V_t(x))^{+}))^{-\frac{\kappa(2+\nu)+8}{8}}(\tilde V_{\gamma[0,t],\tilde t}(V_t(z))-\tilde W_{\gamma[0,t],\tilde t})\notag\\
&\times(\tilde V_{\tilde t}(V_t(z))-\tilde V_{\tilde t}(V_t(y)))^{\frac{\kappa(6+\nu)-16}{8}}(\tilde V_{\gamma[0,t],\tilde t}(V_t(z))-\tilde V_{\gamma[0,t],\tilde t}(W_t))^{-\frac{\kappa}{4}}.
\end{align}
We denote by $\eta$ the $\hSLE_{\kappa'}(\nu)$ curve from $0$ to $\infty$ and denote by $\PP_{\hSLE}$ the probability measure and denote by $\E_{\hSLE}$ the correponding expectation. We define $\tau_\eps$ to be the hitting time of $\gamma$ of the $\eps$-neighbour of $[y,+\infty)$. We still need four Lemmas which correspond to Lemma~\ref{lem::1}, Lemma~\ref{lem::2}, Lemma~\ref{lem::3} and Lemma~\ref{lem::4} in the case $\nu>-2$.

The following lemma is the analog og Lemma~\ref{lem::1}.
\begin{lemma}\label{lem::5}
If $\tilde t=0$, for $t\le \tau_\eps$, we define 
\[N_t:=\int_{y}^{+\infty}M_{t,0}(z)dz.\]
For any bounded measurable function $f$ on the curve space, we have
\[\E_{\hSLE}[f(\eta[0,\tau_\eps])]=\E\left[f(\gamma[0,\tau_\eps])\frac{N_{\tau_\eps}}{N_0}\right].\]
\end{lemma}
\begin{proof}
Note that $N_t$ is the same as the corresponding martingale in Lemma~\ref{lem::1}.
\end{proof}
The following lemma is the analog og Lemma~\ref{lem::2}. Note that in this case, $\tilde\gamma$ can not hit $[z,+\infty)$.
\begin{lemma}\label{lem::6}
Given $\gamma[0,t]$, we denote by $\PP_{\gamma[0,t]}$ the regular conditional probability measure of $\tilde\gamma$ and denote by $\E_{\gamma[0,t]}$ the corresponding expectation. We define
\begin{align*}
M_{t,\tilde\tau}(z):=&\tilde g'_{\gamma[0,t],\tilde\tau}(V_t(z))g'_t(z)(\tilde V_{\tilde \tau}(V_t(z))-\tilde V_{\tilde t}((V_t(x))^{+}))^{-\frac{\kappa(2+\nu)+8}{8}}(\tilde V_{\gamma[0,t],\tilde t}(V_t(z))-\tilde W_{\gamma[0,t],\tilde t})^{\frac{\kappa(6+\nu)-16}{8}}\\&\times(\tilde V_{\gamma[0,t],\tilde t}(V_t(z))-\tilde V_{\gamma[0,t],\tilde t}(W_t))^{-\frac{\kappa}{4}}.
\end{align*}
Then, we have that $\{M_{t,\tilde t\wedge\tilde\tau}\}_{\tilde t \ge 0}$ is a martingale for $\tilde\gamma$ under $\PP_{\gamma[0,t]}$.
\end{lemma}
\begin{proof}
We define $\tilde\tau_\eps(z)$ to be the hitting time of $\tilde\gamma$ at the $\eps$-neighbour of $[z,+\infty)$. By I\'to's formula, we know that $\{M_{t,\tilde t\wedge\tilde\tau_\eps(z)\wedge\tilde\tau}\}_{\tilde t \ge 0}$ is a martingale. Moreover, weighted by $\{\frac{M_{t,\tilde t\wedge\tilde\tau_\eps(z)\wedge\tilde\tau}}{M_{t,0}}\}_{\tilde t \ge 0}$, the law of $g_t(\tilde\gamma)$ has the same law as $\SLE_\kappa\left(-\frac{\kappa}{2};-\frac{\kappa}{4}(2+\nu)-2,k-4+\frac{\kappa}{4}(2+\nu),\kappa\right)$ curve with marked points $x_1^L=W_t$ and $x_1^R=(V_t(x))^+$, $x_2^R=V_t(y)$, $x_3^R=V_t(z)$. As in Lemma~\ref{lem::2}, we denote this curve by $\hat\gamma$.

To show that $\{M_{t,\tilde t\wedge\tilde\tau}\}_{\tilde t \ge 0}$ is a martingale, we will use the same argument as in Lemma~\ref{lem::2}. The main input is that $\hat\gamma$ does not hit $[V_t(z),\infty)$ almost surely. This fact has been obtained from Theorem~\ref{thm::curve} and Lemma~\ref{lem::aux1} for $\hat\gamma$. Thus, by the same argument as in Lemma~\ref{lem::2}, we have that $\{M_{t,\tilde t\wedge\tilde\tau}\}_{\tilde t \ge 0}$ is a martingale and complete the proof.
\end{proof}
Now, we define the probability measure $\LQ_\eps$ to be the probablity measure of $\PP$ weighted by $\frac{\int_{y}^{\infty}M_{\tau_\eps,\tilde\tau}(z)dz}{N_0}$.
The following lemma is the analog of Lemma~\ref{lem::3}.
\begin{lemma}\label{lem::7}
Under the probability measure $\LQ_\eps$, the marginal law of $\gamma[0,\tau_\eps]$ is the same as the law of $\hSLE_{\kappa'}(\nu)$ with force points $x$, $y$ stopped at the hitting time at the $\eps$-neighbour of $[y,\infty)$. The conditional law of $\gamma[0,\tau_\eps]$ can also be described by the following way: We first generate $\tilde\gamma$ under the probability measure $\LQ_\eps$. Denote by $D$ the unbounded connected component of $\HH\setminus\tilde\gamma$. Then, $\gamma$ has the same law as the $\SLE_{\kappa'}$ curve stopped at the hitting time at the $\eps$-neighbour of $[y,\infty)$.
\end{lemma}
\begin{proof}
Note that
\[M_{\tau_\eps,\tilde\tau}(z)=\tilde g'_{\gamma[0,t],\tilde t}(V_t(z))g'_t(z)(\tilde V_{\tilde t}(V_t(z))-\tilde V_{\tilde t}(V_t(y)))^{-\frac{\kappa-4}{2}}(\tilde V_{\gamma[0,t],\tilde t}(V_t(z))-\tilde V_{\gamma[0,t],\tilde t}(W_t))^{-\frac{\kappa}{4}},\]
which is exactly the same as~\eqref{eqn::finallyform}. By the same conputation as in Lemma~\ref{lem::7}, we complete the proof.
\end{proof}
The following lemma is the analog of Lemma~\ref{lem::4}. Suppose $l$ has the same law as 
\\$\SLE_\kappa\left(-\frac{\kappa}{4}(2+\nu)-2,k-4+\frac{\kappa}{4}(2+\nu)\right)$ starting from $x$ with marked point $x_1^R=x^+$, $x_2^R=y$. Denote by $\tau_l$ the hitting time of $l$ at $y$ and denote by $\{g_{l,t}: 0\le t\le \tau_l\}$ the  conformal map associated to $l$. Denote by $V_{l,\cdot}$ the corresponding Loewner evolution.
\begin{lemma}\label{lem::8}
Recall that we denote by $\tilde\tau$ the hitting time of $\tilde\gamma$ at $y$. Then, suppose that $f$ is a bounded and measurable function on the curve space $\LC$, we have
\[\LQ_\eps[f(\tilde\gamma[0,\tilde\tau])]=\frac{1}{\mathcal{Z}}\E_l[f(l[0,\tau_l])(g'_{l,\tau_l}(0))^{\frac{3\kappa-8}{16}}\one_{\{l\cap(-\infty,0]=\emptyset\}}],\]
where $\mathcal{Z}$ is a constant. 
\end{lemma}
\begin{proof}
First of all, by~\cite[Theorem 3]{SchrammWilsonSLECoordinatechanges}, $l$ has the same law as $\SLE_\kappa\left(-\frac{\kappa}{4}(2+\nu)-2\right)$ curve from $x$ to $y$ stopped at its hitting time at $(y,+\infty)$ with marked point $x_1^R=x^+$. Thus, we have almost surely, $l$ ends at $y$ and $l$ does not hit $\R\setminus \{x,y\}$.

For $t<\tau_l$, we define
\begin{align*}
R_t(z):=&g'_{l,t}(z)g'_{l,t}(0)^{\frac{3\kappa-8}{16}}(V_{l,t}(z)-W_{l,t})(V_{l,t}(z)-V_{l,t}(y))^{\frac{\kappa(6+\nu)-16}{8}}(V_{l,t}(z)-V_{l,t}(x^+))^{-\frac{\kappa(2+\nu)+8}{8}}\\
&\times (V_{l,t}(z)-V_{l,t}(0))^{-\frac{\kappa}{4}}(V_{l,t}(0)-W_{l,t})^{-\frac{1}{2}}(V_{l,t}(0)-V_{l,t}(x))^{\frac{\kappa(2+\nu)+8}{16}}(V_{l,t}(z)-V_{l,t}(y))^{-\frac{\kappa(6+\nu)-16}{16}}.
\end{align*}
We define $\tau_{l,\eps}(z,0)$ to be the first time that $l$ hits the $\eps$-neighbour of $(-\infty,0]\cup [z,+\infty)$. By I\'to's formula, we have $\{R_{t\wedge\tau_{l,\eps}(z,0)\wedge\tau_{l}}\}_{t\ge 0}$ is a martingale for $l$. 
By Girsanov's theorem, weighted by $\left\{\frac{R_{t\wedge\tau_{l,\eps}(z,0)\wedge\tau_{l}}(z)}{R_0(z)}\right\}_{t\ge 0}$, the law of $l[0,\tau_{l,\eps}(z,x)\wedge\tau_{l}]$ is same as the law of  
\\$\SLE_\kappa\left(-\frac{\kappa}{2};-\frac{\kappa}{4}(2+\nu)-2,\kappa-4+\frac{\kappa}{4}(2+\nu),\kappa\right)$ curve with  marked points $x_1^L=0$ and $x_1^R=x^+$, $x_2^R=y$, $x_3^R=z$, which stopped at the corresponding stopping time.

By letting $t\to\infty$, we can define 
\[R_{\tau_{l}}(z):=g_{l,\tau_l}'(z)g_{l,\tau_l}'(0)^{\frac{3\kappa-8}{16}}(V_{l,\tau_l}(z)-V_{l,\tau_l}(y))^{\frac{\kappa-4}{2}}(V_{l,\tau_l}(z)-V_{l,\tau_l}(0))^{-\frac{\kappa}{4}}(V_{l,\tau_l}(0)-V_{l,\tau_l}(y))^{\frac{4-\kappa}{4}}.\]
Then, by the same argument as in Lemma~\ref{lem::4}, we have that $\{R_{t\wedge\tau_l}(z)\}_{t\ge 0}$ is a martingale. Comparing $R_{\tau_{l}}(z)$ with~\eqref{eqn::auxmart}, the remaining computation is exactly the same as the computation in the proof of Lemma~\ref{lem::4}. This completes the proof.
\end{proof}
\begin{proof}[Proof of Theorem~\ref{thm::reversibility} when $\frac{\kappa'}{2}-6<\nu<-2$]
The proof is exactly the same as the proof of the case $\nu>-2$. The main difference is, in the case that $\frac{\kappa'}{2}-6<\nu<-2$, $l$ has the same law as $\SLE_\kappa\left(-\frac{\kappa}{4}(2+\nu)-2\right)$ curve form $y$ to $x$ stopped at its hitting time at $(y,+\infty)$. We need the time-reversibility of the $\SLE_\kappa\left(-\frac{\kappa}{4}(2+\nu)-2\right)$ curve, which is the conclusion of Theorem~\ref{thm::slerever} ($\rho_1^L=0$, $\rho_1^R=-\frac{\kappa}{4}(2+\nu)-2$). This completes the proof.
\end{proof}  
